Complexity of Finding Stationary Points of Nonsmooth Nonconvex Functions

We provide the first non-asymptotic analysis for finding stationary points of nonsmooth, nonconvex functions. In particular, we study the class of Hadamard semi-differentiable functions, perhaps the largest class of nonsmooth functions for which the chain rule of calculus holds. This class contains examples such as ReLU neural networks and others with non-differentiable activation functions. We first show that finding an $\epsilon$-stationary point with first-order methods is impossible in finite time. We then introduce the notion of $(\delta, \epsilon)$-stationarity, which allows for an $\epsilon$-approximate gradient to be the convex combination of generalized gradients evaluated at points within distance $\delta$ to the solution. We propose a series of randomized first-order methods and analyze their complexity of finding a $(\delta, \epsilon)$-stationary point. Furthermore, we provide a lower bound and show that our stochastic algorithm has min-max optimal dependence on $\delta$. Empirically, our methods perform well for training ReLU neural networks.

==> inexact_nesterov.tex <==

\section{Inexact Nesterov}
Inexact oracle setting: given any $y \in \R$, we are able to evaluate an inexact gradient $g_y$ such that 
\begin{equation}
	\E[g_y]=\nabla f(y) \quad \text{ and } \quad \E[\Vert g_y - \nabla f(y)\Vert^2 ] \leq C, 
\end{equation}
where $C$ is a constant (typically in the form $\epsilon^{1.5}$).

\begin{proposition}
	Consider Nesterov's method with inexact gradient update, 
	\begin{align*}
		&x_{k+1} = y_k - \frac{1}{L} g_k, \\
		&v_{k+1} = x_{k+1} + \frac{1-\alpha_k}{\alpha_k} (x_{k+1}-x_k),\quad \text{ with } \alpha_k^2 = (1-\alpha_k)\alpha_{k-1}^2 + q\alpha_k \text{ and } q = \frac{\mu}{L}\\
		&y_{k+1} = \eta_{k+1} v_{k+1} + (1-\eta_{k+1}) x_{k+1}, \quad \text{ with } \eta_{k+1} = \frac{\alpha_{k+1} - q}{1-q}.
	\end{align*}
	Then, for any $k \geq 1$
	\begin{equation}
		\E \left [ f(x_{k+1}) -f^* + \frac{L\alpha_k^2}{2} \Vert v_{k+1} - x^* \Vert^2 \right ] \leq (1-\alpha_k) \left ( f(x_{k}) -f^* + \frac{L\alpha_{k-1}^2}{2} \Vert v_{k} - x^* \Vert^2 \right ) + \frac{C}{L}
	\end{equation}
\end{proposition}
\begin{proof}
First, by $L$-smoothness,
\begin{equation}
	f(x_{k+1}) \leq f(y_k) + \langle \nabla f(y_k), x_{k+1}-y_k \rangle + \frac{L}{2} \Vert x_{k+1} -y_k \Vert^2. 
\end{equation}	
Moreover, by strong convexity, for any $z$, we have 
\begin{equation}
	f(y_k) + \langle \nabla f(y_k), z-y_k \rangle + \frac{\mu}{2} \Vert z -y_k \Vert^2 \leq f(z). 
\end{equation}
Adding up the two inequalities yields,
\begin{equation}
	f(x_{k+1}) \leq f(z) +  \langle \nabla f(y_k), x_{k+1}-z \rangle+ \frac{L}{2} \Vert x_{k+1} -y_k \Vert^2 -\frac{\mu}{2} \Vert z -y_k \Vert^2. 
\end{equation}	
Note that
\begin{align*}
	\langle \nabla f(y_k), x_{k+1}-z \rangle & = \langle g_k, x_{k+1}-z \rangle + \langle \nabla f(y_k)-g_k, x_{k+1}-z \rangle \\
	& = L \langle y_k -x_{k+1}, x_{k+1}-z \rangle + \langle \nabla f(y_k)-g_k, x_{k+1}-z \rangle,
\end{align*}
and when $z$ is adapted to the $k$-th filtration, 
\begin{equation*}
	\E[\langle \nabla f(y_k)-g_k, x_{k+1}-z \rangle] = \E[\langle \nabla f(y_k)-g_k, -\frac{1}{L} g_k ] = \frac{1}{L} \E [ \Vert \nabla f(y_k)-g_k \Vert^2 ]
\end{equation*}
Thus, 
\begin{equation}
	\E[f(x_{k+1})] \leq f(z) +  \E \left [ L \langle x_{k+1}-y_k, z-x_{k+1} \rangle + \frac{L}{2} \Vert x_{k+1} -y_k \Vert^2 \right ] -\frac{\mu}{2} \Vert z -y_k \Vert^2 + \frac{C}{L}. 
\end{equation}
Now take $z_k = \alpha_k x^* + (1-\alpha_k) x_k$, then 
\begin{align*}
	& f(z_k) \leq \alpha_k f^* + (1-\alpha_k) f(x_k) - \frac{\mu \alpha_k(1-\alpha_k)}{2} \Vert x_k -x^* \Vert^2, \\
	& z_k - x_{k+1} = \alpha_k (x^* - v_{k+1}).
\end{align*}
Therefore,
\begin{align*}
	& \E \left [ f(x_{k+1}) -f^* + \underbrace{\frac{L\alpha_k^2}{2} \Vert v_{k+1} - x^* \Vert^2}_{ = \frac{L}{2} \Vert z_k -x_{k+1} \Vert^2 } \right ] \\
\leq \quad  & (1-\alpha_k) (f(x_k)-f^*) + \E \left [ \frac{L}{2}\Vert z_k -x_{k+1} \Vert^2 + L \langle x_{k+1}-y_k, z_k-x_{k+1} \rangle + \frac{L}{2} \Vert x_{k+1} -y_k \Vert^2 \right ] \\
 & -\frac{\mu}{2} \Vert z_k -y_k \Vert^2- \frac{\mu \alpha_k(1-\alpha_k)}{2} \Vert x_k -x^* \Vert^2 + \frac{C}{L} \\
 = \quad  & (1-\alpha_k) (f(x_k)-f^*) + \frac{L-\mu}{2} \Vert z_k -y_k \Vert^2- \frac{\mu \alpha_k(1-\alpha_k)}{2} \Vert x_k -x^* \Vert^2 + \frac{C}{L}
\end{align*}
It remains to prove that for any $k\geq 1$,
\begin{equation}\label{eq:zk-yk}
	\frac{L-\mu}{2} \Vert z_k -y_k \Vert^2 \leq (1-\alpha_k) \frac{L\alpha_{k-1}^2}{2} \Vert v_k -x^* \Vert^2 + \frac{\mu \alpha_k(1-\alpha_k)}{2} \Vert x_k -x^* \Vert^2
\end{equation}
In fact,
\begin{align*}
	& \frac{L-\mu}{2} \Vert z_k -y_k \Vert^2  \\
= \quad & \frac{L-\mu}{2} \Vert \alpha_k x^* + (1-\alpha_k) x_k - \eta_k v_k - (1-\eta_k) x_k \Vert^2 \\
= \quad & \frac{L-\mu}{2} \Vert (\alpha_k-\eta_k) (x^*-x_k) + \eta_k (x^*- v_k)  \Vert^2 \\
= \quad & \frac{(L-\mu)\alpha_k^2}{2} \left \Vert (1- \frac{\eta_k}{\alpha_k}) (x^*-x_k) + \frac{\eta_k}{\alpha_k} (x^*- v_k) \right  \Vert^2  \\
\leq \quad &  \frac{(L-\mu)\alpha_k^2}{2} \left ( (1- \frac{\eta_k}{\alpha_k}) \Vert x^*-x_k \Vert^2 + \frac{\eta_k}{\alpha_k} \vert x^*- v_k \Vert^2  \right ) \\
=  &  \frac{(L-\mu)\alpha_k(\alpha_k-\eta_k)}{2} \Vert x^*-x_k \Vert^2 + \frac{(L-\mu)\alpha_k \eta_k}{2} \Vert x^*- v_k \Vert^2  
\end{align*}
We remark that 
\begin{align*}
& \frac{(L-\mu)\alpha_k(\alpha_k-\eta_k)}{2} = \frac{L}{2}(1-q)\alpha_k (\alpha_k - \frac{\alpha_k-q}{1-q})= \frac{L}{2} \alpha_k q(1-\alpha_k) = \frac{\mu \alpha_k(1-\alpha_k)}{2}, \\
&	\frac{(L-\mu)\alpha_k \eta_k}{2} = \frac{L}{2} (1-q)\alpha_k  \frac{\alpha_k-q}{1-q} = \frac{L}{2} \alpha_k (\alpha_k-q) = \frac{L}{2} (1-\alpha_k) \alpha_{k-1}^2. 
\end{align*}
We remark that when $k=0$, 
\begin{equation}
	 z_0 - y_0  = \alpha_0 x^* + (1-\alpha_0) x_0 -y_0 = \alpha_0(x^* -x_0)
\end{equation}
Then we have 
\begin{equation}
	\E \left [ f(x_{1}) -f^*+ \frac{L\alpha_0^2}{2} \Vert v_{1} - x^* \Vert^2 \right] \leq (1-\alpha_0)(f(x_0)-f^*)+ \frac{L \alpha_0(\alpha_0-q)}{2} \Vert x_0 -x^* \Vert^2 + \frac{C}{L}
\end{equation}

\end{proof}
As a.corollary, we have 
\begin{corollary} \label{cor:inexact-agd}
	For any $k\geq 0$, 
	\begin{align*}
		&\E \left [ f(x_{k+1}) -f^* + \frac{L\alpha_k^2}{2} \Vert v_{k+1} - x^* \Vert^2 \right ]  \\
		\leq \quad &\prod_{j=1}^k (1-\alpha_j) \left ( (1-\alpha_0)(f(x_0)-f^*)+ \frac{L \alpha_0(\alpha_0-q)}{2} \Vert x_0 -x^* \Vert^2 \right ) + E_k,
	\end{align*}
	where the error 
	\begin{equation}
		E_k = \frac{C}{L} \left ( 1 + (1-\alpha_k) + (1-\alpha_k)(1-\alpha_{k-1}) + \cdots + \prod_{j=1}^k (1-\alpha_j) ) \right).
	\end{equation}
	In particular, if $\alpha_0 =\sqrt{q}$, then $\alpha_k = \sqrt{q}$ for all $k$. Thus,
	$$E_k \leq \frac{C}{\sqrt{\mu L}},$$
	and 
	$$ \E \left [ f(x_{k+1}) -f^* + \frac{\mu}{2} \Vert v_{k+1} - x^* \Vert^2 \right ]  \leq \left (1-\sqrt{\frac{\mu}{L}} \right )^{k+1} \left ( f(x_0)-f^* + \frac{\mu}{2} \Vert x_0-x^* \Vert^2 \right ) + \frac{C}{\sqrt{\mu L}}$$
\end{corollary}










==> sections/subgaussian.tex <==
\section{Proof of Theorem~\ref{thm:sub}}\label{proof:sub}

\begin{algorithm}[tb]
	\caption{ Sub-Gaussian INGD }\label{algo:sub}
	\begin{algorithmic}
		\FOR{$k = 1, 2, ..., K$} 
% 		\STATE $\mathcal{G} = \{\nabla f(x_k)\}, g = \nabla f(x_k)$
		\STATE Call oracle $S_1$ times and compute $\sim, m_{k,1} = \frac{1}{S_1}\sum_{s=1}^{S_1}\mathbb{O}(x_k, \vec{0})$
		\STATE  Call oracle $S_3$ times and compute $f_{k,1}, \sim = \frac{1}{S_3}\sum_{s=1}^{S_3} \mathbb{O}(x_k, \vec{0})$

		\FOR{$j = 1, ..., J$}
		\STATE Update $x_{k+1} = x_k - \delta \frac{m_{k,j}}{\|m_{k,j}\|} $
		\STATE Call oracle $S_2$ times and compute $\sim , g_{k,j} = \frac{1}{S_2}\sum_{s=1}^{S_2} \mathbb{O}(y_s, -m_{k,j})$,
		\STATE \quad where $y_s$ is sampled uniformly from $ [x_k, x_{k+1}]$
		\STATE \textbf{if} {$\|m_{k,j}\| \le \epsilon/2$ or $\|g_{k,j}\| \le \epsilon/2$} \textbf{then} return $x_k$
		\STATE Call oracle $S_3$ times and compute $f_{k,j+1}, \sim = \frac{1}{S_3}\sum_{s=1}^{S_3} \mathbb{O}(x_{k+1}, \vec{0})$
		\IF {$f_{k,j+1} - f_{k,j} \ge \frac{-\delta \epsilon}{2}$}
		\STATE $m_{k,j+1} = \beta m_{k,j} + (1-\beta) g_{k,j} $, with $\beta = \frac{2L^2 - \|m_{k,j}\|\epsilon/2}{2(\|m_{k,j}\|^2 + L^2 - \|m_{k,j}\|\epsilon/2)}$.
		\ELSE
		\STATE break j-loop.
		\ENDIF		
		\ENDFOR
		\ENDFOR
		
		\STATE \textbf{return} $x_K$
	\end{algorithmic}
\end{algorithm}


By sub-Gaussian properties, we show in Lemma~\ref{lemma:sub-gaus} that if  $S_1 = 12\frac{\sigma_g^2}{\epsilon^2}\log(\frac{L\Delta}{\delta\epsilon\gamma})$, $S_2 = 12\frac{\sigma_f^2}{\epsilon^2\delta^2}\log(\frac{L\Delta}{\delta\epsilon\gamma})$, $S_3 = 12\frac{\sigma_g^2 + L^2}{\epsilon^2}\log(\frac{L\Delta}{\delta\epsilon\gamma})$, $KJ \le \frac{16\Delta L^2}{\delta\epsilon^3}$ then with probability $1-\gamma$, for all $k\le K, j \le J$, conditioned on $x_k$

\begin{align}\label{eq:accuracy}
    \|m_{k, 1} - \E[m_{k,1}|x_k]\| \le \frac{\epsilon}{8} \nonumber \\
    |f_{k, j} - f(x_k)| \le \frac{\delta\epsilon}{16}\nonumber\\
    \|g_{k, j} - \E[g_{k,j}|m_{k,j}]\| \le \frac{\epsilon}{8}
\end{align}

Conditioned on the above event, we show in Lemma~\ref{lemma:gaus-inner} bound that the inner j-loop either finds a $(\delta,\epsilon)$ stationary point or the objective function decreases by $\frac{\delta \epsilon}{4}$.

Since the objective function value can decrease at most $K=\frac{4\Delta}{\delta \epsilon}$ times , the total oracle complexity is bounded by

\begin{align*}
    KJ(S_1 + S_2 + S_3) = \frac{384L^2}{\epsilon^3\delta}(\frac{\sigma_g^2+ L^2}{\epsilon^2}+ \frac{\sigma_f^2}{\epsilon^2\delta^2})\log(\frac{L\Delta}{\delta\epsilon\gamma}).
\end{align*}


\subsection{Technical Lemmas}
\begin{lemma}\label{lemma:sub-gaus}
If we set $S_1 = 12\frac{\sigma_g^2}{\epsilon^2}\log(\frac{L\Delta}{\delta\epsilon\gamma})$, $S_2 = 12\frac{\sigma_f^2}{\epsilon^2\delta^2}\log(\frac{L\Delta}{\delta\epsilon\gamma})$, $S_3 = 12\frac{\sigma_g^2 + L^2}{\epsilon^2}\log(\frac{L\Delta}{\delta\epsilon\gamma})$, then the inequalities in \eqref{eq:accuracy} holds with probability at least $1- \gamma$.
\end{lemma}
\begin{proof}
 We first show that $ \|g_{k, j} - \E[g_{k,j}|m_{k,j}]\|$ is $4\sqrt{L^2 + \sigma^2}$ sub-Gaussian. Given a randomly sampled $y_s \sim [x_{k}, x_{k}- \frac{\delta\|m_{k, j}}{m_{k,j}}]$, denote the $g^*$ in Assumption~\ref{assump} as $g^*(y_s)$. Denote $g := \E[g^*(y_s)|m_{k, j}] = \E[g_{k,j}|m_{k,j}]$. By Assumption~\ref{assump} in the sub-Gaussian case, we know that for any $v$ such that $\|v\| = 1$,
\begin{align*}
    \E[\exp(\frac{\iprod{g(y_s)-g^*(y_s)}{v}^2}{\sigma_g^2})] \le 2. 
\end{align*}
By boundedness that $\|g^*(y)\| \le L$, we know that 
\begin{align*}
    \E[\exp(\frac{\iprod{g^*(y_s) - g}{v}^2}{4L^2})] \le 2. 
\end{align*}
Consequently, we know that when $\psi = 4\sqrt{L^2 + \sigma^2}$, we have that conditioned on $m_{k,j}$,
\begin{align*}
    \E[\exp(\frac{\iprod{g(y_s)-g}{v}^2}{\psi^2})] &\le \E[\exp(\frac{2\iprod{g(y_s)-g^*(y_s)}{v}^2}{\psi^2}) \exp(\frac{2\iprod{g-g^*(y_s)}{v}^2}{\psi^2})] \\
    &\le \E[\E[\exp(\frac{2\iprod{g(y_s)-g^*(y_s)}{v}^2}{\psi^2})|y_s] \exp(\frac{2\iprod{g-g^*(y_s)}{v}^2}{\psi^2})]\\
    &\le \E[\sqrt{2} \exp(\frac{2\iprod{g-g^*(y_s)}{v}^2}{\psi^2})] \le 2
\end{align*}
Hence, $g(y_s)-g$ is $\psi-$sub-Gaussian conditioned on $x_{k, j}$. The theorem follows by applying Hoeffding inequality.


\end{proof}

\begin{lemma}\label{lemma:gaus-inner}
Under the assumption in \eqref{eq:accuracy}, the inner j-loop either finds a $(\delta,\epsilon)$ stationary point or the objective function decreases by $\frac{\delta \epsilon}{4}$ after $J = \frac{4L^2}{\epsilon^2}$
\end{lemma}
If $f_{k, j+1} \le f_{k, j} - \frac{-\delta \epsilon}{2}$, then we know that 
\begin{align*}
    f(x_{k+1}) - f(x_k) &= ( f(x_{k+1}) - f_{k, j+1}) + (f_{k, j+1} - f_{k, j}) + (f_{k, j} - f(x_k))\\
    &\le \frac{\delta \epsilon}{16} + \frac{-\delta \epsilon}{2} + \frac{\delta \epsilon}{16} \le \frac{-3\delta \epsilon}{8}.
\end{align*}
Then the loop breaks and the Lemma is true. Otherwise, assume that $f_{k, j+1} > f_{k, j} - \frac{-\delta \epsilon}{2}$ for all $k$ in the loop. Then we know that
\begin{align*}
    \|m_{k,j+1}\|^2 &= \|\beta m_{k,j} + (1-\beta)g_{k, j}\|^2] \le \beta^2 \|m_{k,j}\|^2 + (1-\beta)^2 L^2 + 2\beta(1-\beta)\iprod{g_{k, j}}{m_{k,j}} \\
    &=\beta^2 \|m_{k,j}\|^2 + (1-\beta)^2 L^2 + 2\beta(1-\beta)\iprod{g_{k, j} - \E[g_{k, j}|m_{k, j}]}{m_{k,j}} + 2\beta(1-\beta)\iprod{\E[g_{k, j}|m_{k, j}]}{m_{k,j}} \\
    &=  \beta^2 \|m_{k,j}\|^2 + (1-\beta)^2 L^2 + 2\beta(1-\beta)(\frac{\|m_{k,j}\|\epsilon}{8}+\frac{-3\|m_{k,j}\|\epsilon}{8}) \\
    &= \beta^2(\|m_{k,j}\|^2 + L^2 - \|m_{k,j}\|\epsilon/2) +  \beta (-2L^2 + \|m_{k,j}\|\epsilon/2) + L^2
\end{align*}

The third equality follows by 
\begin{align*}
\iprod{\E[g_{k, j}|m_{k, j}]}{-\frac{\delta m_{k,j}}{\|m_{k,j}\|}} = \E[\iprod{g_{k,j}}{x_{k+1} - x_k}|m_{k, j}] = \int f'(\gamma(t), x_{k+1} - x_k) dt
\end{align*}
The rest of the proof is the same as Lemma~\ref{lemma:det-while}.
